Optimizing Locally Differentially Private Protocols

Protocols satisfying Local Differential Privacy (LDP) enable parties to collect aggregate information about a population while protecting each user's privacy, without relying on a trusted third party. LDP protocols (such as Google's RAPPOR) have been deployed in real-world scenarios. In these protocols, a user encodes his private information and perturbs the encoded value locally before sending it to an aggregator, who combines values that users contribute to infer statistics about the population. In this paper, we introduce a framework that generalizes several LDP protocols proposed in the literature. Our framework yields a simple and fast aggregation algorithm, whose accuracy can be precisely analyzed. Our in-depth analysis enables us to choose optimal parameters, resulting in two new protocols (i.e., Optimized Unary Encoding and Optimized Local Hashing) that provide better utility than protocols previously proposed. We present precise conditions for when each proposed protocol should be used, and perform experiments that demonstrate the advantage of our proposed protocols.

==> attack.tex <==
% !TEX root = rappor.tex
We now study the effect of the Instantaneous randomized response in the RAPPOR approach.


Using RAPPOR's decoding method, one uses each reporting after the instantaneous randomized response step.  This is less accurate than the user directly sending the result after the Permanent randomized response step.  
\says{Ninghui}{Maybe we can add a quantitative measure of this on the level of frequency of things can be recovered.}
 %Note that against an attacker who can 
 %Adding this step hurts utility without improving privacy against an attacker who .  

\subsection{The Attack}

Consider the following game: The Challenge chooses two values $x$ and $x'$, then derive the two permanent random response bitvectors $B_1$ and $B_1'$, and two Instantaneous random response vector from $B_1$, $B_2^{(1)}$ and $B_2^{(2)}$, and one $B_2'$, from $B_1'$.  The Challenger flip an unbiased coin and get results $b$; if $b=1$, it sends $B_2^{(1)}$ and $B_2^{(2)}$, and if $b=0$, it sends $B_2^{(1)}$ and $B_2'$.  

The high-level intuition is that with high probability, $B_1$ and $B_1'$ will have many bits that are different.  For example, using RAPPOR with the following parameters: $f=1/2$, $p=0.75$, $q=0.25$, 128-bit vectors, two hash functions.  We expect that on average $B_1$ and $B_1'$ each have about $33$ bits being $1$.  Since these are random, we would expect that $B_1$ and $B_2$ to have more than $50$ bits that are different.  

Two bit vectors from the same are expected to have $80$ bits that are the same.  Standard deviation is $5.47$.  Two bit vectors from different users are expected to have $63$ bits that are the same.

\says{Ninghui}{This means that the distinguishability won't be very sharp when there are many users.  Maybe we will exclude this part.  }

\subsection{Experimental Results}
\says{Ninghui}{Do the following experiments.  Use RAPPOR with $f=1/2$, $p=0.75$, $q=0.25$, 128-bit vectors, two hash functions.  Generate 1 million responses.  }


==> cand.tex <==
In some scenarios,
to enumerate the possible answers may be computationally infeasible
(e.g., find the frequent length-$\ell$ strings),
thus it is a challenge to find the frequent items (heavy hitters).
 
In this section,
we go through methods for selecting frequent candidates over a large domain.

\subsection{Filtering Candidates during Joint Estimation}
The first method we can use is the joint estimation method,
presented in Section \ref{sec:multi}.
However, these methods enumerate all possible candidates, 
thus we need to filter infrequent ones during the process.










==> experiment.tex <==
% !TEX root = rappor.tex

%LDP is useful to learn unknown distributions.
%It helps to better understand and estimate knowledge we were not allowed to learn previously.
%For instance, to deal with large scale online guessing,
%website administrators can disable weak passwords (those appear frequently) once the distribution of passwords is known.
%
%However, it is not easy to learn user's password
%(available password datasets are all get from accidental leakage).
%Typically users won't be willing to share their passwords.

We now study the application of LDP protocols to password modeling as a case study.  We present Private Password Oracle (\ldpsys).  Using \ldpsys, each user can report information based on her password in a way that satisfies LDP, and the aggregator is able to build a password model to identify frequent (i.e., weak) passwords.  A large website can, e.g., deploys such a system that identifies weak passwords specific for users of the site and ban the usage of these passwords in the future.

%, Locally Differentially Private Probabilistic Password Models. \says{tianhao}{a better name is desired.}\ldpsys{} privately aggregates password data, and uses this aggregated data to measure password strength. Our empirical results demonstrate that LDP protocol can indeed help us to build improved domain-specific password models. The challenge lies in the fact that domain of possible passwords is very large, while the number of users is relatively small.

%We open sourced the code for experiments \cite{support}. Datasets are provided on request.

\subsection{System Description}
%We first provide the overview of \ldpsys, then we go over the details of the building blocks of \ldpsys.

We observe that many large-scale real-world password datasets already exist.  However, a privacy-preserving technique to build password models is still desirable.  Patterns in creating passwords vary between speakers of different languages~\cite{Ma2014study,Li2014}.  Also, each website tends to have frequent passwords specific to it, e.g., ``rockyou'' is the $8$-th most frequent password in the Rockyou dataset.  Therefore, our goal is to enable the extraction of population-specific frequent passwords and combine them with models built using generic datasets.

\mypara{Hash Blacklist.}  One goal is to build a blacklist of frequent passwords while satisfying LDP.  Because the space of all passwords is very large, we first hash each password to a length-$20$ bit string, and then have each user report the hash value using the \OLH protocol (i.e., we have $d=2^{20}$).  Note that in this process each password is hashed twice, the first hash function is shared by all users and the aggregator, and hashes each password to a value in $[2^{20}]$. The second hashing step is done inside the \OLH protocol, and each user uses a different hash function.

The aggregator can then estimate the frequency of each of $2^{20}$ hashes.  If a password has a hash that is identified as frequent, then that password is banned.  Due to collisions, some passwords may be banned even if they are not frequent.  Banning, e.g., 100 passwords obtained this way means that a password that is not frequent still has a $\frac{100}{2^{20}} \approx \frac{1}{10,000}$ probability of being banned.  Increasing the hash length can further reduce this probability, at the cost of increasing aggregation cost for the aggregator.  (The user-side cost does not change.)
Such a blacklist also contains the frequencies, and thus gives an estimated probability of each password in the list.

\mypara{Significance Test.}
Given the aggregation result, we need to filter those likely to be contributed from noise. Similar to \rappor{}, for each value, we compare its estimation with a threshold
$$T = \Phi^{-1}\left(1-\frac{0.05}{d}\right) \sqrt{\frac{4 e^\epsilon }{(e^\epsilon-1)^2}\cdot n},$$
where $d$ is the domain size, $\Phi^{-1}$ is the inverse of the cumulative density function of standard normal distribution, and the term inside the square root is the variance.
When $\epsilon=6$ and $d=2^{20}$, this yields $T= 0.533\sqrt{n}$.

\mypara{Private Markov Model.}  With a few million users, the number of passwords that would be detected by the blacklist approach above is typically less than $100$.  We thus also build a Markov model while satisfying LDP, by extracting $n$-gram frequencies.  Each user randomly chooses an $n$-gram and reports it.  Based on the observation that the vast majority of users use lower-case letters and digits in their passwords, we report only $n$-grams consisting of letters and digits.

The aggregator computes estimation for each possible $n$-gram (there are $36^n$ such $n$-grams).  We use the same significance test method as the above to identify frequent $n$-grams.  To build a Markov model, we need to estimate frequencies of all other $n$-grams as well.  We compute an estimated total frequency for all non-frequent $n$-grams and divide this number evenly among all them.  The estimation is done by assuming that the $n$-gram frequencies follow the Zipf's distribution.
Specifically, let $D$ be the set of all $n$-grams, and $D_s$ be the set of those with estimated frequency above the threshold, the total frequency for all other $n$-grams is estimated as
$$\sum_{i\in D\backslash D_s}\tilde{c}(i)=\sum_{i\in D_s}\tilde{c}(i)\cdot\frac{\sum_{i=|D_s|+1}^{|D|}\frac{1}{i}}{\sum_{i = 1}^{|D_s|} \frac{1}{i}}.$$
With these $n$-gram frequencies, we can construct a Markov model using techniques in~\cite{Castelluccia2012,Ma2014study}.  More specifically, we prepend $n-1$ start symbols to each password, and use the length normalization technique in~\cite{Ma2014study}, that is, the total probabilities of passwords of the same length is first estimated, and then distributed among all passwords of the same length.

One important parameter is which $n$ to use for $n$-grams.  When $n$ is too small  (such as $n=2$), we are not extracting patterns specific to a dataset.  When $n$ is large, the frequency of $n$-grams decreases, while at the same time the number of candidates increases, pushing higher the threshold, causing relatively few $n$-grams to be discovered as frequent.  In our experiments, we use $n=4$, which appears to work better than other choices.

%\says{ninghui}{too much detail}
%Users are partitioned into four groups. For $G = 1, 2, 3$, users in group $G$ report based on the first $G$ characters of the password, and users in the last group report based on any length-$4$ substring (password length suffices guaranteed by data cleansing). Note that this step still satisfies $\epsilon$-LDP.

\mypara{Partition Population vs. Partition Privacy Budget?}
We want to learn both a blacklist and a password model while satisfying $\epsilon$-LDP.  More generally, when one needs to answer two questions while satisfying $\epsilon$-LDP, one can either split the privacy budget $\epsilon$ into two portions $\epsilon=\epsilon_1+\epsilon_2$ and use one portion for each question; or one can (randomly) choose one question to answer.  An intriguing question is which way provides better utility?  In the non-local setting, there is typically little difference between the two approaches, as most algorithms have accuracy scaling with $N\epsilon$, where $N$ is the total number of users.  Interestingly, this is not the case for LDP.

%In LDP we often want to aggregate the answers to {\em multiple} questions. For example, our goal is to train two models $M_h$ (Hash Blacklist) and $M_m$ (Markov Model). There are two natural approaches to aggregate answers to multiple questions in local differential privacy. For example, to answer two questions we could partition the population into two groups and use the first (resp. second) group to answer the first question (resp. second question) using a LDP protocol with privacy parameter $\epsilon$. Alternatively, each user could partition his privacy budget and participate in separate LDP protocols for each parameters with privacy parameters $\epsilon_1$ and $\epsilon_2=\epsilon-\epsilon_1$. Which strategy is better?

The variance and the significant thresholds provide a good guideline for this question.  We can compute the significance threshold, $T_1$, from using half of the privacy budget but the total population, with $T_2$ from using the total privacy budget but half the population.  When $T_1 > 2T_2$, splitting the population is better than splitting the privacy budget and vice versa, since we expect to get double the count with the whole population, compared with using half.
In \OLH, with $\epsilon=4$, we have $T_1 \approx 4.36 T_2$, and with $\epsilon=6$, we have $T_1 \approx 6.65 T_2$.  This suggests that splitting the population is better than splitting the privacy budget.

\begin{comment}
In \OLH,
$$\sigma^2=n\cdot\frac{4e^\epsilon}{(e^\epsilon-1)^2}, T=Q\frac{2\sqrt{ne^{\epsilon}}}{e^{\epsilon}-1}$$
If we partition $\epsilon$ into halves, and users answer both questions,
the threshold $T_1=Q\frac{2\sqrt{ne^{\epsilon/2}}}{e^{\epsilon/2}-1}$,
however, if we divide the population,
we have the threshold $T_2=Q\frac{\sqrt{2ne^{\epsilon}}}{e^{\epsilon}-1}$.
Let $\epsilon=4$, we have $T_1=8.5\sqrt{n}Q$, while $T_2=3.9\sqrt{n}Q$ (compared with $T=2.8\sqrt{n}Q$ if we answer only one question). This means we can potentially identify more domains.
This is also an evidence we shouldn't divide privacy budget and repeatedly answer questions.
\end{comment}

\mypara{Putting Things Together.}  In \ldpsys, the population is partitioned so that each user reports either a hash or a randomly-chosen $4$-gram of the password satisfying LDP. A private Markov chain model (using $4$-grams) $M_m$ and a private Hash Blacklist $M_h$ are constructed based on users' reports. \ldpsys also uses an additional model $M_p$, learned using publicly available data, the Rockyou dataset.  Given a password $pwd$, each model outputs a probability. Their average is taken as the prediction.

%In $M_h$, users are required to report a perturbed hash of his password. Passwords that are not captured by $M_m$ will be effectively captured by $M_h$.

%Markov chain models may occasionally miss frequent passwords that do not come from natural language, e.g. ``147258369'' or ``1qaz2wsx'' (these are adjacent patterns on the keyboard). To capture such passwords we also use LDP to maintain a blacklist of hashes of frequent passwords.

%\ldpsys{} takes an LDP protocol as primitive, and train three models:

\begin{comment}
\ldpsys{} enjoys flexibility of using any LDP protocol as the primitive,
any combination of partition to train models,
and any heuristic to aggregate predictions by different models.
For different tasks, the optimal choice may be different.

The training dataset is partitioned into half to train both $M_m$ and $M_h$.
We trained an additional Backoff Markov model $M_p$ on Rockyou, and take a weighted average of predictions output by all three models to extract our final result.


\says{Jeremiah}{Consider moving next two segments below (Markov Chain + Significance Test and Model-Fitting Smoothing) to appendix}
\mypara{Markov chain.}
Markov chains are often used to model natural language. Given a (natural language) string $s_1,\ldots,s_{i+o}$, a Markov chain model of order $o$ specifies the distribution of the next character
$$ \Pr{s_{i+o}|s_1s_2\ldots s_{i+o-1}}=\Pr{s_{i+o}|s_{i}s_{i+1}\ldots s_{i+o-1}}$$
Then to evaluate likelihood of a whole string $S = s_1s_2\ldots s_l$, we just multiply each length-$(o+1)$ segment:
$$\Pr{s_1s_2\ldots s_l}=\Pr{s_1}\cdot\Pr{s_2|s_1}\cdots\Pr{s_l|s_{l-o}s_{l-o+1}\ldots s_{l-1}}$$

During the process of training, we may not observe all possible segments. Moreover, due to the constraint of privacy, we may not estimate frequency of some segment reliably. We thus use standard significance test and model-fitting smoothing, as described below.

One challenge with using Markov models for password distributions is that a string ``password'' will be evaluated to be less frequent than ``passwor'', which is never the case in reality. To overcome challenges like this, we use distribution based normalization. Specifically,
$$\Pr{s_1s_2\ldots s_l}_{l} = \Pr{s_1s_2\ldots s_l}\cdot\Pr{|S|=l}$$

We use Markov chain of order $3$.
Users are partitioned into four groups $G=1,2,3$ and $4$. For $G = 1, 2, 3$,
users in group $G$ report based on the first $G$ characters of their password. Users in the last group $G=4$ report based on any length-$4$ substring (password length suffices guaranteed by data cleansing). User reports are always subject to the constraints of $\epsilon$-LDP.

For the estimations that are below the threshold, we fit a Zipf's distribution.
Specifically, assume $D_s$ is the set of significant estimations that are above the threshold,
the total amount of the estimations below the threshold should be
$$\sum_{i\in D\backslash D_s}\tilde{c}(i)=\sum_{i\in D_s}\tilde{c}(i)\cdot\frac{\sum_{i\in [|D_s|]}\frac{1}{i}}{\sum_{i\in [|D| - |D_s|]}\frac{1}{i}}$$
we assume all of them are equally likely.
\end{comment}



\begin{comment}
\mypara{How to Partition?}
With several questions, each with different domain sizes,
we have demonstrated that partition the population will be better,
now a natural question is how to partition the groups.
Because of the privacy constraints, the number of reliable estimation is less than square root of the population size.
For the questions with smaller domain size, a smaller amount of users suffices. For example, the first group in the noisy Markov chain model only reports the first character of their passwords using LDP. Since the domain $d=36$  is small (lower case letters + digits), $20K$ users suffice for this task.
Sometimes, with limited amount of users, we cannot reliably estimate all the domains (especially for the last group in noisy Markov chain model, we need more than $36^8$ users).

In the experiment, we first partition the users into halves, to train the noisy Markov chain model and Hash Blacklist model, respectively. For the noisy Markov chain model,
we put $\frac{1}{60}$, $\frac{1}{30}$, and $\frac{1}{15}$ fraction of the population to the first three groups, and put the rest to the last group.
Note that this partition does not rely on the underlying dataset. We did not put much effort to optimize this partition.
\end{comment}


\subsection{Experimental Setup}

We evaluate \ldpsys{} via experiments.  The goal of constructing blacklists and password models is to identify weak passwords so that forbidding them can yield more secure password distributions.  We use the Normalized $\beta$-Residual Strength Graph ($\beta$-NRSG) introduced in~\cite{yang2016comparing} to compare models built from \ldpsys{} with models built only from the public dataset.

The $\beta$-NRSG graph illustrates the strength of weakest passwords left once we ban some passwords according to some model.  It is computed with a test dataset.
 %Each model will rank passwords.  When
Specifically, each algorithm corresponds to a curve in the graph. Each point $(x, y)$ means that, after banning $x$ passwords in the test dataset, the residual strength of the passwords, $\log\left(\frac{\beta}{\sum_{i=1}^{\beta}\Pr{w_i}}\right)$,
is $y$, where $\Pr{w_i}$ is the frequency of the $i$-th weakest password that is not banned in the testing dataset according to the model.
Intuitively, residual strength measures the strength of the $\beta$ weakest (remaining) passwords in the dataset, as measured by the $\beta$-success-rate, proposed by Bozta\c{s}~\cite{Boztas1999} and Bonneau~\cite{Bonneau2012}.  Given a $\beta$-success-rate $p$, we use $-\log_2 p$ to turn this into an effective key-length metric.  Thus, higher $y$ means stronger password distribution.  If model $X$ results in a curve above that from model $Y$, this means that using $X$ one is able to improve password security by banning fewer (other) passwords in the dataset (than using $Y$ does), i.e., inflicting less inconvenience for users using these other banned passwords.

%The normalized version of $\beta$-RSG is slightly different from $\beta$-RSG in that a value $x$ means $x$ weakest password in the testing dataset according to the algorithm.  \says{Jeremiah}{I don't understand the last sentence}

\mypara{Datasets.}
We use the following four password datasets that are publicly available:
The \textbf{RockYou} dataset~\cite{PasswordsList} contains over 32 million passwords. It is leaked by the Website in Dec. 2009.
To demonstrate the context difference, we use three Chinese datasets to evaluate:
The \textbf{CSDN} dataset includes about 6 million passwords for the
Chinese Software Developer Network (CSDN), a popular IT portal and a
community for software developers in China~\cite{CSDN1}.
The \textbf{Duduniu} dataset contains about 16 million passwords for a paid online gaming site in China.
The \textbf{178} datasets includes about 10 million passwords for another gaming website in China.
We performed data cleansing operations suggested in~\cite{yang2016comparing}.
More specifically, we use DBSCAN~\cite{ester1996density} to remove likely fake account/password pairs in the datasets.
For the Chinese datasets, three quarters are used for private learning, and a quarter is used for evaluating.

 %Then, we restrict the passwords to be composed of only digits and lower-case characters.
 %After cleansing, Rockyou, CSDN, Duduniu and 178 contain 27, 5, 7, and 7 million passwords respectively.

\mypara{Baselines.} In our experiments we use a model $M_p$ trained on RockYou (primarily English speaking users) as our baseline for comparison. RockYou is intended to model publicly available datasets in our experiment. Because there are no privacy constraints we build two models on Rockyou: a Backoff Markov chain model (see~\cite{Ma2014study} for details), and a Blacklist model, which simply rank passwords according to their frequencies in Rockyou. We evaluate these two baseline methods on Chinese password datasets to capture the scenario where publicly available password data may not be representative of the particular demographics at another organization.
 %This Markov model $M_p$ may also be used by \ldpsys. Our goal is to see if we can improve performance by training an additional Markov Model $M_m$ and hash blacklist $M_h$ using LDP.

\begin{comment}
\mypara{Discussion of Privacy Budget.}
In \ldpsys, users only need to report a perturbed segment of their passwords
(i.e., a length-4 string) in $M_m$. Thus, even if the adversary guesses the segment correctly, the probability he guesses the {\em entire} password is limited. For $M_h$, even if the adversary get to know the user's password hash, he cannot find a unique pre-image of the hash since we hash passwords to a smaller domain $d=2^{20}$. The best strategy of the adversary is to try all the frequent passwords. Thus, it is possible to use a slightly larger privacy budget. In the experiment, we use $\epsilon = 4, 6, 8$. The higher the $\epsilon$, the better the result, but sometimes a smaller $\epsilon$ suffices.
\end{comment}

\begin{figure*}[t]
%	\captionsetup[subfigure]{aboveskip=-1pt,belowskip=-1pt}
	\centering

	\subfigure[178, $\beta=1$]{
		\label{fig:residual_178_178_qstd_residual_1}
		\includegraphics[width=0.63\columnwidth]{figure/password/residual/178_178_qstd_residual_1}
	}
	\subfigure[CSDN, $\beta=1$]{
		\label{fig:residual_csdn_csdn_qstd_residual_1}
		\includegraphics[width=0.63\columnwidth]{figure/password/residual/csdn_csdn_qstd_residual_1}
	}
	\subfigure[Duduniu, $\beta=1$]{
		\label{fig:residual_duduniu_duduniu_qstd_residual_1}
		\includegraphics[width=0.63\columnwidth]{figure/password/residual/duduniu_duduniu_qstd_residual_1}
	}
	\centering
	\subfigure[178, $\beta=10$]{
		\label{fig:residual_178_178_qstd_residual}
		\includegraphics[width=0.63\columnwidth]{figure/password/residual/178_178_qstd_residual}
	}
	\subfigure[CSDN, $\beta=10$]{
		\label{fig:residual_csdn_csdn_qstd_residual}
		\includegraphics[width=0.63\columnwidth]{figure/password/residual/csdn_csdn_qstd_residual}
	}
	\subfigure[Duduniu, $\beta=10$]{
		\label{fig:residual_duduniu_duduniu_qstd_residual}
		\includegraphics[width=0.63\columnwidth]{figure/password/residual/duduniu_duduniu_qstd_residual}
	}
	\vspace{-0.2cm}
		\caption{
		Normalized Residual Strength Graph: \ldpsys with different $\epsilon$ values compared against Rockyou Markov chain and Rockyou Black List.  The $x$ axis is number of banned passwords in the dataset; the $y$ axis is the $\beta$-residual strength.}
	\label{fig:residual_exp}
\end{figure*}
\begin{figure*}[!htb]
	\centering
	\vspace{-0.2cm}
	\subfigure[178, $\beta=1$]{
		\label{fig:residual_178_178_qstd_residual_vary_model_1}
		\includegraphics[width=0.63\columnwidth]{figure/password/residual/178_178_qstd_residual_1_vary_model}
	}
	\subfigure[CSDN, $\beta=1$]{
		\label{fig:residual_csdn_csdn_qstd_residual_vary_model_1}
		\includegraphics[width=0.63\columnwidth]{figure/password/residual/csdn_csdn_qstd_residual_1_vary_model}
	}
	\subfigure[Duduniu, $\beta=1$]{
		\label{fig:residual_duduniu_duduniu_qstd_residual_vary_model_1}
		\includegraphics[width=0.63\columnwidth]{figure/password/residual/duduniu_duduniu_qstd_residual_1_vary_model}
	}
	\centering
	\subfigure[178, $\beta=10$]{
		\label{fig:residual_178_178_qstd_residual_vary_model}
		\includegraphics[width=0.63\columnwidth]{figure/password/residual/178_178_qstd_residual_vary_model}
	}
	\subfigure[CSDN, $\beta=10$]{
		\label{fig:residual_csdn_csdn_qstd_residual_vary_model}
		\includegraphics[width=0.63\columnwidth]{figure/password/residual/csdn_csdn_qstd_residual_vary_model}
	}
	\subfigure[Duduniu, $\beta=10$]{
		\label{fig:residual_duduniu_duduniu_qstd_residual_vary_model}
		\includegraphics[width=0.63\columnwidth]{figure/password/residual/duduniu_duduniu_qstd_residual_vary_model}
	}
	\vspace{-0.2cm}
	\caption{
		Normalized Residual Strength Graph: \ldpsys, Markov only, Hash blacklist only, and budget splitting. The $x$ axis is number of banned passwords in the dataset; the $y$ axis is the $\beta$-residual strength.}
	\label{fig:vary_mode_exp}
\end{figure*}
\begin{figure*}[!htb]
	\centering
	\vspace{-0.2cm}
	\subfigure[178, $\beta=1$]{
		\label{fig:residual_178_178_qstd_residual_annoy_1}
		\includegraphics[width=0.63\columnwidth]{figure/password/residual/178_178_qstd_residual_1_annoy}
	}
	\subfigure[CSDN, $\beta=1$]{
		\label{fig:residual_csdn_csdn_qstd_residual_annoy_1}
		\includegraphics[width=0.63\columnwidth]{figure/password/residual/csdn_csdn_qstd_residual_1_annoy}
	}
	\subfigure[Duduniu, $\beta=1$]{
		\label{fig:residual_duduniu_duduniu_qstd_residual_annoy_1}
		\includegraphics[width=0.63\columnwidth]{figure/password/residual/duduniu_duduniu_qstd_residual_1_annoy}
	}
	\centering
	\subfigure[178, $\beta=10$]{
		\label{fig:residual_178_178_qstd_residual_annoy}
		\includegraphics[width=0.63\columnwidth]{figure/password/residual/178_178_qstd_residual_annoy}
	}	
	\subfigure[CSDN, $\beta=10$]{
		\label{fig:residual_csdn_csdn_qstd_residual_annoy}
		\includegraphics[width=0.63\columnwidth]{figure/password/residual/csdn_csdn_qstd_residual_annoy}
	}
	\subfigure[Duduniu, $\beta=10$]{
		\label{fig:residual_duduniu_duduniu_qstd_residual_annoy}
		\includegraphics[width=0.63\columnwidth]{figure/password/residual/duduniu_duduniu_qstd_residual_annoy}
	}
	\caption{
		Residual strength graph: \ldpsys with $\epsilon=4$, Rockyou Markov chain model, Rockyou Black List, and three basic composition policies: Len8, D+L, and Both. The $x$ axis is the percentage of users whose passwords are banned and are thus required to change their passwords.}
	\label{fig:percent_exp}
\end{figure*}

%Experimental Result for 178 Dataset. The left two columns (i.e.,
%Figures~\ref{fig:residual_178_178_qstd_residual_1}, \ref{fig:residual_178_178_qstd_residual_vary_model_1},
%\ref{fig:residual_178_178_qstd_residual}) plot the Normalized Residual Strength Graph.
%Figures~\ref{fig:residual_178_178_qstd_residual_1}, \ref{fig:residual_178_178_qstd_residual_vary_model}, compares Hybrid mode using \OLH{} and Basic RAPPOR as primitives, Rockyou Markov chain model, and Rockyou Blacklist.
%\begin{figure*}[t]
%	\centering
%	\subfigure[178]{
%		\label{fig:residual_178_178_qstd_guess}
%		\includegraphics[width=0.95\columnwidth]{figure/password/residual/178_178_qstd_guess}
%	}
%	\subfigure[CSDN]{
%		\label{fig:residual_178_178_qstd_guess}
%		\includegraphics[width=0.95\columnwidth]{figure/password/residual/csdn_csdn_qstd_guess}
%	}
%	\subfigure[Duduniu]{
%		\label{fig:residual_duduniu_duduniu_qstd_guess}
%		\includegraphics[width=0.95\columnwidth]{figure/password/residual/duduniu_duduniu_qstd_guess}
%	}
%	
%	\caption{Guess Number Graphs}
%	\label{fig:residual_guess_exp}
%\end{figure*}


\subsection{Evaluation Results}
We plot Normalized $\beta$-Residual Strength Graph ($\beta$-NRSG)~\cite{yang2016comparing} for $\beta=1$ and $\beta=10$, comparing the result of \ldpsys{} and baselines. Our results are shown in Figures \ref{fig:residual_exp}, \ref{fig:vary_mode_exp}, and \ref{fig:percent_exp}.

 %\textbf{1. Primitive Comparison.}

Figure~\ref{fig:residual_exp} plots the $1$-NRSG and resp. $10$-NRSG using three datasets: 178, CSDN, and Duduniu.
 %\ref{fig:residual_178_178_qstd_residual_1} (resp. \ref{fig:residual_178_178_qstd_residual})  plots $x$ vs. $1$-NRSG (resp. $10$-NRSG) using the 178 password dataset for evaluation. The RockYou BL plot (solid square) shows the effectiveness of banning the most popular $x$ RockYou passwords. Even if we ban the top $2^{18}$ RockYou passwords the weakest remaining passwords in the 178 dataset only have about $y=8.5$ bits of entropy.
It shows the effect of \ldpsys{} with three privacy budgets $\epsilon=4,6,8$.  On 178, the advantage of \ldpsys over the baseline is quite clear.  For example, using \ldpsys with $\epsilon=6$, just banning enough passwords so that $2^{8}$ passwords in the dataset are banned (incurring a very small inconvenience cost) can raise the bit-strength for $\beta=1$ from the original $6$ to $10$; whereas using just the Rockyou-trained model requires banning more than $2^{18}$ passwords to reach the same strength level.  The advantage of \ldpsys over rockyou model is less pronounced on CSDN and Duduniu, perhaps because their the distribution is closer to Rockyou.   Increasing privacy budget from $4$ to $6$ and from $6$ to $8$ all introduce significant improvements.

\begin{comment}
that the right-most line
We can see that \ldpsys{} results in better
Training a Markov model $M_p$ based on RockYou passwords yields no improvement. However, notice that \ldpsys{} overall improves the residual strength significantly by training additional Markov models $M_m$ and Hash Blacklist $M_h$ with LDP protocols. In this particular plot \ldpsys{} performs best when we use \OLH{} instead of RAP (Basic RAPPOR), but this difference is insignificant in some datasets (e.g., Figure \ref{fig:residual_csdn_csdn_qstd_residual_1}).
\end{comment}

 %\textbf{2. Model Combination Comparison.}
Figure~\ref{fig:vary_mode_exp} compares the performance of \ldpsys against using only hash blacklist, only a probability model, and splitting privacy budget instead of splitting the population.  It clearly shows that \ldpsys, which splits the population, performs better than splitting the privacy budget.  It also shows that training only a Markov model (and does not use a hash blacklist) performs not as well.  Interestingly, constructing only a hash blacklist using the \OLH protocol (and combining the list with a Markov model built from rockyou) performs slightly better than \ldpsys.  This suggests that hash blacklist is also a promising approach and in fact may be more attractive because it is simple to implement.

%\ref{fig:residual_178_178_qstd_residual_vary_model_1} (resp. \ref{fig:residual_178_178_qstd_residual_vary_model})  plots $x$ vs. $1$-NRSG (resp. $10$-NRSG) using the 178 password dataset for evaluation.  Four different model combinations are compared.

%Training a Markov model $M_p$ based on RockYou passwords yields no improvement. However, notice that \ldpsys{} overall improves the residual strength significantly by training additional Markov models $M_m$ and Hash Blacklist $M_h$ with LDP protocols. In this particular plot \ldpsys{} performs best when we use \OLH{} instead of RAP (Basic RAPPOR), but this difference is insignificant in some datasets (e.g., Figure \ref{fig:residual_duduniu_duduniu_qstd_residual_1}).

 %\textbf{3. Comparison with Basic Composition Policies.}
Figure~\ref{fig:percent_exp} compares the effect of \ldpsys and other password modeling approach with that of three basic password composition policies.
Policy ``Len8'' requires each password to be no less than $8$ characters;
policy ``D+L'' requires each password to be composed of both digits and letters;
policy ``Both'' requires both Len8 and D+L.
In Figure~\ref{fig:percent_exp}, we can see that using composition policies, a large number of users will be required to change their passwords, but the residual strength is pretty low.
Policy Both performs better than the other two in terms of residual strength ($y \approx 10$),
but at a cost of inconveniencing more than $80\%$ of the users for 178 and CSDN, and more than $60\%$ of users for duduniu, while Len8 and D+L perform best in terms of usability ($60\%$ of users disturbed) though these policies provide minimal security (e.g., $y\approx 7$, $8$). In contrast, \ldpsys{} improves both usability an security. For example, we can increase $\beta=1$-residual strength to $y > 10$ while affecting no more than $15\%$ of users for all three datasets.
We also note that \ldpsys{} greatly outperforms Rockyou models in 178, somewhat outperforms Rockyou models in Duduniu, and barely outperform Rockyou models in CSDN.

%in from $x=0$ to $x=0.3$, where $30\%$ is arguably a reasonable upper bound on the maximum number of users an organization would be willing to bother to improve password strength.
%In reality, we won't use those policies, because they are banning too many passwords (even so, the residual strength is low).
%$30\%$ would be a reasonable threshold.

\begin{comment}
We use the CSDN, 178, and Duduniu password datasets for evaluation, and we use the Rockyou dataset as the baseline. From the figures, we can see that \ldpsys{} overall improves the residual strength. Specifically, when $\beta = 1$, the baseline gets stuck after $x=5, 3, 1$ on evaluating 178, CSDN, and Duduniu, respectively. That is because some frequent password (e.g., ``147258369'' and ``1qaz2wsx'') in the evaluating dataset is not captured by Rockyou model. With the same model, the performance of the baseline actually depends on the similarity of from the evaluating dataset.
We can see from the results that the statistical distance is big for those datasets.
However, with \ldpsys, the performance is similarly good for all datasets.
This is resulted from both the Hash Blacklist, that captures frequent pattern based passwords,
and the Markov chain model, that captures frequent language based passwords.
Finally, performance does increase with the increase of privacy budget.



\mypara{Datasets.}
We use the following four password datasets that are publicly available:
\textbf{RockYou} dataset~\cite{PasswordsList} contains over 32 million passwords that were leaked in Dec. 2009.
To demonstrate the context difference, we use three Chinese datasets to evaluate:
\textbf{CSDN} dataset includes about 6 million passwords for the
Chinese Software Developer Network (CSDN), a popular IT portal and a
community for software developers in China~\cite{CSDN1}.
\textbf{Duduniu} dataset contains about 16 million passwords for a paid online gaming site in China.
\textbf{178} datasets includes about 10 million passwords for another gaming website in China.
\end{comment}

%Experimental Result for 178 Dataset. The left two columns (i.e.,
%Figures~\ref{fig:residual_178_178_qstd_residual_1}, \ref{fig:residual_178_178_qstd_residual_vary_model_1},
%\ref{fig:residual_178_178_qstd_residual} and \ref{fig:residual_178_178_qstd_residual_vary_model} ) plot the Normalized Residual Strength Graph.
%Figures~\ref{fig:residual_178_178_qstd_residual_1} and \ref{fig:residual_178_178_qstd_residual}, compare Hybrid mode using \OLH{} and Basic RAPPOR as primitives, Rockyou Markov chain model, and Rockyou Black List.
%Figures~\ref{fig:residual_178_178_qstd_residual_vary_model_1} and  \ref{fig:residual_178_178_qstd_residual}, compare Hybrid mode, Hash only mode, Markov chain only mode and Split Privacy (with Hybrid) mode. All plots use \OLH{} as the primitive and $\epsilon=6$.
%The right column (Figure~\ref{fig:residual_178_178_qstd_residual_annoy_1} and \ref{fig:residual_178_178_qstd_residual_annoy} ) plot the residual strength vs percentage of users that are required to change passwords. We compare Hybrid mode with OLH and $\epsilon=4$, Rockyou Markov chain model, Rockyou Black List, and three basic composition policies, i.e., password length should be greater than $8$ (Len8), password should be composed of both digits and letters (D+L), and both.

%	\begin{subfigure}{}
%		\includegraphics[width=0.63\columnwidth]{figure/password/residual/178_178_qstd_residual_1}
%		\caption{178, $\beta=1$}
%		\label{fig:lab0}
%	\end{subfigure}
%\begin{subfigure}[t]{}
%	\centering
%	\includegraphics[width=0.63\columnwidth]{figure/password/residual/178_178_qstd_residual_1}
%	\caption{t = 0.5 s and Re = 100}
%\end{subfigure}
%~
%\begin{subfigure}[t]{}
%	\centering
%	\includegraphics[width=0.63\columnwidth]{figure/password/residual/178_178_qstd_residual_1}
%	\caption{t = 1.0 s and Re = 100}
%\end{subfigure}
%~
%\begin{subfigure}[t]{}
%	\centering
%	\includegraphics[width=0.63\columnwidth]{figure/password/residual/178_178_qstd_residual_1}
%	\caption{t = 1.0 s and Re = 100}
%\end{subfigure}



==> hash.tex <==
\says{tianhao}{this could potentially be the most practical and accuracy protocol}
Bassily and Smith proposed a method that is able to find frequent items from a large domain.
The intuition is to use \protUnary{}, 
and instead of encoding every possible answer 
(domain size $d$, which is infeasible),
they encode $d' = O(poly(n))$ domains.
To set $d'$ large enough (e.g., $d' = n^{1.5}$), 
it is possible to reduce the number of collisions during the process of projection.

The answers are projected by the guidance of hash functions,
thus coding theory is used to recover the value after hashing.

After discovering the frequent domains, 
it is possible to use the current frequency as the result,
or one can use another channel only collecting frequent candidates.

Now we formally describe protocol. 
We start from the simplest version of the protocol,
and then add more (optional) features to improve it.
\begin{protocol}[\protHashS] \label{prot:hash} $\;$\\
	
	\mypara{Reporting.}
	Then user $j$, with answer $a^j\in[d]$, reports $\report^j$, a length-$d'$ vector,
	sampled from the following distribution:
	\begin{align*}
	\mbox{When }i = \mathtt{hash}(a^j): \;&\Pr{\report^{j}_i = 1} = p, \Pr{\report^{j}_i = 0} = q, \\
	\mbox{When }i \neq \mathtt{hash}(a^j): \;
	&\Pr{\report^j_i = 0} = p, \Pr{\report^j_i = 1} = q, \\
	\mbox{where } &p = \frac{e^{\epsilon/2}}{e^{\epsilon/2} + 1}, q = 1-p
	\end{align*}
	Finally the user responses with report $\report^j$ to server. 
	
\mypara{Recovery. (Scaling)} 
The server, after receiving all reports,
rescales to get the estimation of counts for all possible hashes:
Suppose $\tilde{C_i}$ is the true count for hash $i$,
then $\tilde{C_i}\cdot p + (n - \tilde{C_i})\cdot q = \sum_{j}\report^j_i$, 
thus 
\begin{align*}
\tilde{C_i} &= \frac{\sum_{j}I(\report^j_i == 1) - n q}{p-q}
\end{align*}
	
\end{protocol}

The server in this protocol can only estimate the frequency of hashes.
It is possible a hash value results from different original values.
In such cases,
multiple rounds of this protocol (with privacy budget divided) is necessary.

Moreover, to get the original value, coding algorithms are used: 
\begin{definition}[Binary ($d, s, \zeta$)-code] \label{def:code}
	A binary ($d, s, \zeta$)-code is a pair of algorithms ($\mathtt{Enc, Dec}$) where
	$\mathtt{Enc}:[d]\rightarrow[s]$, and $\mathtt{Dec}:[s]\rightarrow[d]$,
	such that up to $\zeta/2$ fraction of errors can be corrected.
\end{definition}

\begin{proposition}
	There exists efficient Binary ($d, s, \zeta$)-code constructions.
\end{proposition}

Formally, the full protocol proceeds as follows:
\begin{protocol}[\protHash] \label{prot:hash2} $\;$\\
	
	\mypara{Reporting Candidates.}
	Then user $j$, with answer $a^j\in[d]$, reports $R^j=\{\report^{j,t}, \reportX^{j,t}\}_{t\in[T]}$, a length-$d'$ vector,
	sampled from the following distribution:
	\begin{align*}
	\forall t\in[T]\\
	\mbox{When }i = &\mathtt{hash}(t, a^j): \;\\
	&\mbox{encode }a^j: e = enc(a^j); \reportX^{j,t}_i\xleftarrow{\$}[s]\\
	&\Pr{\report^{j,t}_i = e_{\reportX^{j,t}_i}} = p, \Pr{\report^{j,t}_i = 1-e_{\reportX^{j,t}_i}} = q, \\
	\mbox{When }i \neq &\mathtt{hash}(t, a^j): \;\\
	&\reportX^{j,t}_i\xleftarrow{\$}[s]\\
	&\Pr{\report^{j,t}_i = 0} = p, \Pr{\report^{j,t}_i = 1} = q, \\
	\mbox{where } &p = \frac{e^{\epsilon/2T+2}}{e^{\epsilon/2T+2} + 1}, q = 1-p
	\end{align*}
	Finally the user responses with report $R^j$ to server. 
	
	\mypara{Identifying Potential Candidates.} 
	The server, after receiving all reports,
	rescales to get the estimation of counts for all codes:
	Suppose $\tilde{C^t_{i,k}}$ is the true count for $k$-th bit of code $i$ in round $t$,
	then $\tilde{C^t_{i,k}}\cdot p + (n/\log s - \tilde{C^t_{i,k}})\cdot q = \sum_{j}I(\reportX^{j,t}_i=k)\report^{j,t}_i$, 
	thus 
	\begin{align*}
	\tilde{C^t_{i,k}} &= \frac{\sum_{j}I(\reportX^{j,t}_i=k\wedge\report^{j,t}_{i} == 1) - n q}{p-q}
	\end{align*}
	Then for each channel $k$ of each round $t$,
	the server first rounds $\tilde{C^t_{i,k}}$ to $0$ (if $\tilde{C^t_{i,k}} < 0$) or $1$ (if $\tilde{C^t_{i,k}}\geq 0$).
	The server then decodes the rounded estimate to get the candidate.
	There are $t\times d'$ candidates, among them, 
	all frequent ones are included with high probability.
	\mypara{Getting Frequencies}
	After getting frequent candidates, 
	the users and server runs an extra round of frequency oracle.
	Using privacy budget of $\epsilon/(T+1)$.
	Which oracle to use depends on the variance.
	
\end{protocol}

\begin{proposition}
	The \protHash{} will identify all frequent candidate with high probability.
\end{proposition}

==> overview.tex <==


test

In this section,
we go through the system architecture of local differential privacy.

There exists a server and multiple users.
The server wants to learn statistics about the users,
but the users would not like to expose their privacy.

The communication channel between the server and any user is secure,
and the users do not collude.

Server wants to obtain aggregated statistics of different answers to a question.
To do so, the server may possibly challenge the user with some message,
and the user will response differentially privately.
On receiving the responses from users,
the server aggregate the data and summary of the data. 

==> sort.tex <==

\label{subsec:sort}
Instead of enumerating all possible answers, 
which is computationally infeasible,
we can enumerate reports from users.

This requires using Protocol \protRandom{} as the frequency oracle.
\says{tianhao}{Which is not good, because variance of \protRandom{} grows with $d$. 
	It is necessary to find out how other methods can be used in the setting below:}
After getting reports from users in the format of a random response,
the server can sort them (either in the form of quick sort or tree-based sort),
and then rescale them. 
Since there are $n$ reports,
there are at most $n$ items after sorting,
and after rescaling,
the unfiltered candidates (appears some times after rescaling) should be less.

==> syn_img.tex <==
\begin{figure*}[t]
	%	\captionsetup[subfigure]{aboveskip=-1pt,belowskip=-1pt}
	\centering
	
	\subfigure[$n=100000,\epsilon=1$]{
		\label{fig:normal_dist_est_e1_n100000}
		\includegraphics[width=0.95\columnwidth]{figure/new/synthetic/normal_dist_est_e1_n100000}
	}
	\subfigure[$n=1000000,\epsilon=1$]{
		\label{fig:normal_dist_est_e1_n1000000}
		\includegraphics[width=0.95\columnwidth]{figure/new/synthetic/normal_dist_est_e1_n1000000}
	}
	\centering
	\subfigure[$n=100000,\epsilon=2$]{
		\label{fig:normal_dist_est_e2_n100000}
		\includegraphics[width=0.95\columnwidth]{figure/new/synthetic/normal_dist_est_e2_n100000}
	}
	\subfigure[$n=1000000,\epsilon=2$]{
		\label{fig:normal_dist_est_e2_n1000000}
		\includegraphics[width=0.95\columnwidth]{figure/new/synthetic/normal_dist_est_e2_n1000000}
	}
	\centering
	\subfigure[$n=100000,\epsilon=4$]{
		\label{fig:normal_dist_est_e4_n100000}
		\includegraphics[width=0.95\columnwidth]{figure/new/synthetic/normal_dist_est_e4_n100000}
	}
	\subfigure[$n=1000000,\epsilon=4$]{
		\label{fig:normal_dist_est_e4_n1000000}
		\includegraphics[width=0.95\columnwidth]{figure/new/synthetic/normal_dist_est_e4_n1000000}
	}
	\centering
	\subfigure[$n=100000,\epsilon=8$]{
		\label{fig:normal_dist_est_e8_n100000}
		\includegraphics[width=0.95\columnwidth]{figure/new/synthetic/normal_dist_est_e8_n100000}
	}
	\subfigure[$n=1000000,\epsilon=8$]{
		\label{fig:normal_dist_est_e8_n1000000}
		\includegraphics[width=0.95\columnwidth]{figure/new/synthetic/normal_dist_est_e8_n1000000}
	}
	\vspace{-0.2cm}
	\caption{
		True and estimated frequency of values of the normal distribution. }
	\label{fig:syn_normal}
\end{figure*}

\begin{figure*}[t]
	%	\captionsetup[subfigure]{aboveskip=-1pt,belowskip=-1pt}
	\centering
	
	\subfigure[$n=100000,\epsilon=1$]{
		\label{fig:exponential_dist_est_e1_n100000}
		\includegraphics[width=0.95\columnwidth]{figure/new/synthetic/exponential_dist_est_e1_n100000}
	}
	\subfigure[$n=1000000,\epsilon=1$]{
		\label{fig:exponential_dist_est_e1_n1000000}
		\includegraphics[width=0.95\columnwidth]{figure/new/synthetic/exponential_dist_est_e1_n1000000}
	}
	\centering
	\subfigure[$n=100000,\epsilon=2$]{
		\label{fig:exponential_dist_est_e2_n100000}
		\includegraphics[width=0.95\columnwidth]{figure/new/synthetic/exponential_dist_est_e2_n100000}
	}
	\subfigure[$n=1000000,\epsilon=2$]{
		\label{fig:exponential_dist_est_e2_n1000000}
		\includegraphics[width=0.95\columnwidth]{figure/new/synthetic/exponential_dist_est_e2_n1000000}
	}
	\centering
	\subfigure[$n=100000,\epsilon=4$]{
		\label{fig:exponential_dist_est_e4_n100000}
		\includegraphics[width=0.95\columnwidth]{figure/new/synthetic/exponential_dist_est_e4_n100000}
	}
	\subfigure[$n=1000000,\epsilon=4$]{
		\label{fig:exponential_dist_est_e4_n1000000}
		\includegraphics[width=0.95\columnwidth]{figure/new/synthetic/exponential_dist_est_e4_n1000000}
	}
	\centering
	\subfigure[$n=100000,\epsilon=8$]{
		\label{fig:exponential_dist_est_e8_n100000}
		\includegraphics[width=0.95\columnwidth]{figure/new/synthetic/exponential_dist_est_e8_n100000}
	}
	\subfigure[$n=1000000,\epsilon=8$]{
		\label{fig:exponential_dist_est_e8_n1000000}
		\includegraphics[width=0.95\columnwidth]{figure/new/synthetic/exponential_dist_est_e8_n1000000}
	}
	\vspace{-0.2cm}
	\caption{
		True and estimated frequency of values of the exponential distribution. }
	\label{fig:syn_exp}
\end{figure*}
